Direct quantification of topological protection in symmetry-protected photonic edge states at telecom wavelengths

Topological on-chip photonics based on tailored photonic crystals (PhC) that emulate quantum valley Hall effects has recently gained widespread interest due to its promise of robust unidirectional transport of classical and quantum information. We present a direct quantitative evaluation of topological photonic edge eigenstates and their transport properties in the telecom wavelength range using phase-resolved near-field optical microscopy. Experimentally visualizing the detailed sub-wavelength structure of these modes propagating along the interface between two topologically non-trivial mirror-symmetric lattices allows us to map their dispersion relation and differentiate between the contributions of several higher-order Bloch harmonics. Selective probing of forward and backward propagating modes as defined by their phase velocities enables a direct quantification of topological robustness. Studying near-field propagation in controlled defects allows to extract upper limits to topological protection in on-chip photonic systems in comparison to conventional PhC waveguides. We find that protected edge states are two orders of magnitude more robust as compared to conventional PhC waveguides. This direct experimental quantification of topological robustness comprises a crucial step towards the application of topologically protected guiding in integrated photonics, allowing for unprecedented error-free photonic quantum networks.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
